Constrained Reinforcement Learning Has Zero Duality Gap

Autonomous agents must often deal with conflicting requirements, such as completing tasks using the least amount of time/energy, learning multiple tasks, or dealing with multiple opponents. In the context of reinforcement learning~(RL), these problems are addressed by (i)~designing a reward function that simultaneously describes all requirements or (ii)~combining modular value functions that encode them individually. Though effective, these methods have critical downsides. Designing good reward functions that balance different objectives is challenging, especially as the number of objectives grows. Moreover, implicit interference between goals may lead to performance plateaus as they compete for resources, particularly when training on-policy. Similarly, selecting parameters to combine value functions is at least as hard as designing an all-encompassing reward, given that the effect of their values on the overall policy is not straightforward. The later is generally addressed by formulating the conflicting requirements as a constrained RL problem and solved using Primal-Dual methods. These algorithms are in general not guaranteed to converge to the optimal solution since the problem is not convex. This work provides theoretical support to these approaches by establishing that despite its non-convexity, this problem has zero duality gap, i.e., it can be solved exactly in the dual domain, where it becomes convex. Finally, we show this result basically holds if the policy is described by a good parametrization~(e.g., neural networks) and we connect this result with primal-dual algorithms present in the literature and we establish the convergence to the optimal solution.

==> figures/fig_Coarse.tex <==
%!TEX root = root.tex

\begin{tikzpicture}
	\pgfplotsset{select coords between index/.style 2 args={
	    x filter/.code={
	        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
	        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
	    }
	}}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		ymode=log,
		tick scale binop=\times,
		%title style={yshift=-1ex},
		%xlabel near ticks,
		%ylabel near ticks,
		minor y tick num=0,
		minor x tick num=1,
		%ytick={0,0.2,0.4,...,1},
		%title={},
		xlabel={Parametrization Size ($d$)},
		ylabel={Duality Gap},
		ylabel near ticks,
		width=\columnwidth, 
		height=0.45\columnwidth, 
		xmin=1,xmax=5,ymin=0.001,ymax=1,
		grid=both,
		legend style={
			at={(0.98,0.06)}, 
			anchor=south east, 
			legend cell align=left
			}
	]
	
	\addplot [select coords between index={0}{0},
		color=red,only marks,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarseD.dat};

	\addplot [select coords between index={1}{1},
		color=blue,only marks,mark options={blue,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarseD.dat};

	\addplot [select coords between index={2}{2},
		color=green,only marks,mark options={green,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarseD.dat};

	\addplot [select coords between index={3}{3},
		color=orange,only marks,mark options={orange,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarseD.dat};

	\addplot [select coords between index={4}{4},
		color=cyan,only marks,mark options={cyan,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarseD.dat};

	\addplot [black,dashed,thick,no marks]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarseD.dat};

					
\end{axis}
\end{tikzpicture}

==> figures/fig_CoarseIteration.tex <==
%!TEX root = root.tex
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		ymode=log,
		tick scale binop=\times,
		%title style={yshift=-1ex},
		%xlabel near ticks,
		%ylabel near ticks,
		minor y tick num=0,
		minor x tick num=1,
		%ytick={0,0.2,0.4,...,1},
		%title={},
		xlabel={Iteration ($k$)},
		ylabel={Duality Gap},
		ylabel near ticks,
		width=\columnwidth, 
		height=0.45\columnwidth, 
		xmin=0,xmax=100000,ymin=0.001,ymax=1,
		grid=both,
		legend columns=5,
		legend style={
			font=\scriptsize,
			at={(0.5,1.1)}, 
			anchor=south,
			legend cell align=left
			}
	]
	\addplot [color=red,solid,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarse1.dat};
	\addlegendentry{$d=1$};
	
	\addplot [color=blue,solid,thick,mark=none,mark options={blue,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarse2.dat};
	\addlegendentry{$d=2$};
	
	\addplot [color=green,solid,thick,mark=none,mark options={green,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarse3.dat};
	\addlegendentry{$d=3$};
	
	\addplot [color=orange,solid,thick,mark=none,mark options={orange,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarse4.dat};
	\addlegendentry{$d=4$};
	
	\addplot [color=cyan,solid,thick,mark=none,mark options={cyan,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPGCoarse5.dat};				
	\addlegendentry{$d=5$};

\end{axis}
\end{tikzpicture}

==> figures/fig_Gap.tex <==
%!TEX root = root.tex
				
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		ymode=log,
		tick scale binop=\times,
		%title style={yshift=-1ex},
		%xlabel near ticks,
		%ylabel near ticks,
		minor tick num=1,
		%title={},
		xlabel={Iteration ($k$)},
		ylabel={Duality Gap},
		ylabel near ticks,
		width=\columnwidth, 
		height=0.75\columnwidth, 
		xmin=0,xmax=1000000,ymin=0,ymax=1,
		grid=both,
		legend style={
			at={(0.96,0.96)}, 
			anchor=north east, 
			legend cell align=left
			}
	]
	
	\addplot [color=red,solid,thick,mark=none,mark options={red,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGap.dat};
		\addlegendentry{Duality Gap};
	
	\addplot [color=blue,solid,thick,mark=none,mark options={blue,solid}]
		table[x index=0,y index=1, col sep=comma]{figures/data/dataGapPG.dat};	
		\addlegendentry{Duality Gap (PG)};		
	
\end{axis}
\end{tikzpicture}


==> figures/fig_map.tex <==
%!TEX root = root.tex
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		minor tick num=1,
		%xtick={1,3,...,15},	
		%ytick={1,3,...,15},
		xtick={0.5,2.5,...,14.5},
		xticklabels ={},
		%xticklabels ={1,3,...,15},
		ytick={0.5,2.5,...,14.5},
		%yticklabels ={1,3,...,15},
		yticklabels ={},
		extra x ticks={1,3,...,15},			
		extra x tick labels={},        	
		extra y ticks={1,3,...,15},			
		extra y tick labels={},     
        extra tick style={
            grid=both,
        },					
		%title={},
		width=0.8\columnwidth, 
		height=0.8\columnwidth, 
		xmin=0,xmax=15,ymin=0,ymax=15,
		%grid=both,
%		legend columns=3,
%		legend style={
%			font=\scriptsize,
%			at={(0.94,0.98)}, 
%			anchor=north east, 
%			legend cell align=left
%			}
	]
	
	\draw [draw=cyan,fill=cyan!25] (10,10) rectangle (60,60);
	\draw [draw=orange,fill=orange!25] (10,10) rectangle (50,50);
	\draw [draw=green,fill=green!25] (10,10) rectangle (40,40);
	\draw [draw=blue,fill=blue!25] (10,10) rectangle (30,30);
	\draw [draw=red,fill=red!25] (10,10) rectangle (20,20);

	
	\draw [draw=black,fill=black] (0,0) rectangle (10,150);
	\draw [draw=black,fill=black] (0,0) rectangle (150,10);
	\draw [draw=black,fill=black] (140,0) rectangle (150,150);
	\draw [draw=black,fill=black] (0,140) rectangle (150,150);
	
	\draw [draw=black,fill=black] (60,0) rectangle (90,30);
	\draw [draw=black,fill=black] (60,40) rectangle (90,110);
	\draw [draw=black,fill=black] (60,120) rectangle (90,140);
	
	\draw [draw=gray,fill=gray!50] (20,120) rectangle (30,130);
	\draw [draw=gray,fill=gray!50] (120,120) rectangle (130,130);

	%\draw [draw=none,fill=red!50] (60,110) rectangle (90,120);
	\draw [draw=red,fill=red!50] (60,110) rectangle (70,120);
	\draw [draw=red,fill=red!50] (70,110) rectangle (80,120);
	\draw [draw=red,fill=red!50] (80,110) rectangle (90,120);
	
	%\draw [draw=green,fill=green!50] (60,30) rectangle (90,40);
	\draw [draw=blue,fill=blue!50] (60,30) rectangle (70,40);
	\draw [draw=blue,fill=blue!50] (70,30) rectangle (80,40);
	\draw [draw=blue,fill=blue!50] (80,30) rectangle (90,40);

	\addplot [color=blue,solid,thick,mark=*,mark options={blue,solid}]
		table[x index=2,y index=1, col sep=comma]{figures/data/safe.dat};

	\addplot [color=red,solid,thick,mark=*,mark options={red,solid}]
		table[x index=2,y index=1, col sep=comma]{figures/data/unsafe.dat};		
	


\end{axis}
\end{tikzpicture}

